Quantum Prudent Contracts with Applications to Bitcoin

Smart contracts are cryptographic protocols that are enforced without a judiciary. Smart contracts are used occasionally in Bitcoin and are prevalent in Ethereum. Public quantum money improves upon cash we use today, yet the current constructions do not enable smart contracts. In this work, we define and introduce quantum payment schemes, and show how to implement prudent contracts -- a non-trivial subset of the functionality that a network such as Ethereum provides. Examples discussed include: multi-signature wallets in which funds can be spent by any 2-out-of-3 owners; restricted accounts that can send funds only to designated destinations; and "colored coins" that can represent stocks that can be freely traded, and their owner would receive dividends. Our approach is not as universal as the one used in Ethereum since we do not reach a consensus regarding the state of a ledger. We call our proposal prudent contracts to reflect this. The main building block is either quantum tokens for digital signatures (Ben-David and Sattath QCrypt'17, Coladangelo et al. Crypto'21), semi-quantum tokens for digital signatures (Shmueli'22) or one-shot signatures (Amos et al. STOC'20). The solution has all the benefits of public quantum money: no mining is necessary, and the security model is standard (e.g., it is not susceptible to 51\% attacks, as in Bitcoin). Our one-shot signature construction can be used to upgrade the Bitcoin network to a quantum payment scheme. Notable advantages of this approach are: transactions are locally verifiable and without latency, the throughput is unbounded, and most importantly, it would remove the need for Bitcoin mining. Our approach requires a universal large-scale quantum computer and long-term quantum memory; hence we do not expect it to be implementable in the next few years.

==> macros.tex <==
%auto-ignore

\usepackage[draft=false]{hyperref}

\RequirePackage{etex}
\ifnum\sigconf=0\usepackage{authblk}\fi \usepackage{silence} %authbulk must loaded before the silence package!!
\usepackage[modulo]{lineno}
\usepackage{amsthm,amssymb,amsfonts,color,paralist,url,ifdraft,mathrsfs,thm-restate,comment,bbold,booktabs,fullpage}


\usepackage[utf8]{inputenc} \usepackage[autostyle=false, style=english]{csquotes} \MakeOuterQuote{"}

%csquotes after inputenc
\usepackage[T1]{fontenc}
\ifnum\sigconf=0
    \ifnum \shownomenclature=1
        \usepackage[refpage,prefix]{nomencl}
        \newcommand*{\nom}[3]{#2\nomenclature[#1]{#2}{#3}} 
        \makenomenclature
        % the following part makes the nomenclature to be a section rather than a section*. It also gives it a label. In the beginning, I had a solution which was based on the following url, but it stopped working, and that's why it is commented out: https://tex.stackexchange.com/questions/124608/how-to-format-the-name-of-a-nomenclature
        %\xpatchcmd{\thenomenclature}{
        %\section*{\nomname}}{% Replace it by the following
        %\section{\nomname}\label{sec:nomenclature}
        %}{\typeout{Success!}}{\typeout{Failure}}
        
        %since the previous solution didn't work, we simply redefine the command itself. See here for the original command: https://github.com/borisveytsman/nomencl/blob/master/nomencl.dtx
        \makeatletter
        \def\thenomenclature{%
            \providecommand*{\listofnlsname}{\nomname}%
      
        
            \section{\nomname}
            \label{sec:nomenclature}    
            \if@intoc\addcontentsline{toc}{section}{\nomname}\fi%
        
      
            \nompreamble
            \if@nomentbl
                \let\itemOrig=\item
                \def\item{\gdef\item{\\}}%
                \expandafter\longtable\expandafter{\@nomtableformat}
                \else
                \list{}{%
                  \labelwidth\nom@tempdim
                  \leftmargin\labelwidth
                  \advance\leftmargin\labelsep
                  \itemsep\nomitemsep
                  \let\makelabel\nomlabel}%
            \fi
        }
        \makeatother 
    \fi
    
    %\usepackage[draft=false,pageanchor]{hyperref}
    %\def\pagedeclaration#1{, \hyperlink{page.#1}{page\nobreakspace#1}} %This is needed for the nomenclature
    \usepackage{doi}

    \usepackage%[final]
    {graphicx}
\fi


 %\usepackage{mathtools} \mathtoolsset{showonlyrefs} %the mathtools way does not work nicely with sigconf. I *think* aotunum works in all cases.
%\ifdraft{\usepackage{showlabels}}{} %must be after use package{hyperref}.

%\usepackage[refpage,prefix]{nomencl} \newcommand*{\nom}[2]{#1\nomenclature{#1}{#2}} \makenomenclature
%\usepackage[displaymath,textmath,sections,graphics,floats]{preview}
%\RequirePackage{silence}
\WarningFilter{l3regex}{This package is obsolete }

\usepackage [ lambda,advantage , operators , sets , adversary , landau , probability , notions , logic ,ff, mm,primitives , events , complexity , asymptotics , keys]{cryptocode}
%the following commands are defined by crptocode. Define these ourselves if needed: \newcommand{\poly}{\mathrm{poly}} \newcommand{\prob}[1]{\Pr[ #1 ]} \newcommand{\norm}[1]{\left\| #1 \right\|} \newcommand{\RR}{\mathbb{R}} \newcommand{\FF}{\mathbb{F}} \newcommand{\CC}{\mathbb{C}} \newcommand{\NN}{\mathbb{N}}\DeclarePairedDelimiter\ceil{\lceil}{\rceil} \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\renewcommand{\verify}{\ensuremath{\mathsf{verify}}} 


%\renewcommand{\sfdefault}{phv}
%\renewcommand{\rmdefault}{ptm}

\ifdraft{\newcommand{\authnote}[3]{{\color{#3} {\bf  #1:} #2}}}{\newcommand{\authnote}[3]{}}
\newcommand{\note}[1]{{\color{red}#1}}
%Example for how this should be used, in main file:
\newcommand{\snote}[1]{\authnote{Shai}{#1}{purple}}


\newcommand{\CNOT}{\mathrm{CNOT}}
\newcommand{\defeq}{\stackrel{\mathrm{def}}{=}}

\newcommand{\const}{\mathrm{const}}

\newcommand{\bra}[1]{\langle #1 \vert}
\newcommand{\ket}[1]{\vert #1 \rangle}
\newcommand{\ketbra}[1]{\vert #1 \rangle \langle #1 \vert}
\newcommand{\braket}[2]{\langle #1 \vert #2 \rangle}
\newcommand{\conjugate}[1]{#1^{\dagger}}
\newcommand{\tensor}{\otimes}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\transpose}[1]{#1^{\mathsf{T}}}
\ifdraft{\linenumbers}{}

\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\E}{\mathbb{E}}

%\PreviewMacro*\onote
%\PreviewMacro*\nom
%\PreviewMacro*\ifdraft
%\DeclareMathOperator*{\E}{\scalerel*{\mathbb{E}}{\textstyle\sum}}


\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%document specific
\usepackage{algorithm,algorithmicx,algpseudocode}
\usepackage[normalem]{ulem}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sY}{\mathcal{Y}}
\newcommand{\sR}{\mathcal{R}}
\newcommand{\inj}{J}
\newcommand{\Es}[1]{\textsc{E}_{#1}}
\newcommand{\dset}{G}
\newcommand{\BQP}{\textsf{BQP}}
\renewcommand{\supp}{\textsc{Supp}}
\newcommand{\decrypt}{\ensuremath{\mathsf{decrypt}}}
\newcommand{\encrypt}{\ensuremath{\mathsf{encrypt}}}
\newcommand{\ds}{\ensuremath{\mathsf{DS}}}
\newcommand{\tm}{\ensuremath{\mathsf{TM}}}
\newcommand{\stamp}{
 {\mathchoice
  {\includegraphics[height=1.8ex]{RubberStamp}}
  {\includegraphics[height=1.8ex]{RubberStamp}}
  {\includegraphics[height=1.2ex]{RubberStamp}}
  {\includegraphics[height=0.9ex]{RubberStamp}}
 }
}
%\newcommand{\keygen}{\ensuremath{\mathsf{key\textit{-}gen}}}
%\newcommand{\sign}{\ensuremath{\mathsf{sign}}}
%\newcommand{\verify}{\ensuremath{\mathsf{verify}}}


\usepackage{tikz}
\usetikzlibrary{arrows,chains,matrix,positioning,scopes}
%
\makeatletter
\tikzset{join/.code=\tikzset{after node path={%
\ifx\tikzchainprevious\pgfutil@empty\else(\tikzchainprevious)%
edge[every join]#1(\tikzchaincurrent)\fi}}}
\makeatother
%
\tikzset{>=stealth',every on chain/.append style={join},
         every join/.style={->}}
\tikzstyle{labeled}=[execute at begin node=$\scriptstyle,
   execute at end node=$]
%
\ifnum\sigconf=0
    \usepackage[capitalise]{cleveref} %Incompatible with showonlyrefs
    \crefname{Game}{Game}{Games}
\fi

%\usepackage{autonum}%must be loaded after cleveref. Sometimes causes bugs. The alternative is incomaptible with cleveref:
 %\usepackage{mathtools} \mathtoolsset{showonlyrefs} %the mathtools way does not work nicely with sigconf. I *think* aotunum works in all cases. In any case, showonlyrefs does not work with cleveref.
\ifnum\sigconf=0
    \newtheorem{theorem}{Theorem} 
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{definition}[theorem]{Definition}
    \newtheorem{example}[theorem]{Example}
    \newtheorem{conjecture}[theorem]{Conjecture}
\fi 
  \newtheorem{claim}[theorem]{Claim}
  \newtheorem{fact}[theorem]{Fact}
  \newtheorem*{theorem*}{Theorem}
  \newtheorem*{lemma*}{Lemma}
  \newtheorem*{corollary*}{Corollary}
  \newtheorem*{proposition*}{Proposition}
  \newtheorem*{claim*}{Claim}
  
  \theoremstyle{definition}
  \newtheorem{openproblem}[theorem]{Open Problem}
  \theoremstyle{remark}
  \newtheorem{remark}[theorem]{Remark}

  \theoremstyle{plain}
  \renewcommand{\qedsymbol}{$\square$}

\theoremstyle{plain}
\newcounter{Game} 
\setcounter{Game}{0}
\newenvironment{game}[1][htb]
    {
    %\floatname{algorithm}{Game}% Update algorithm name
    %\refstepcounter{Game}%to call the Game pointer. Currently the problem is that caption command by default calls the algorithm pointer. For the moment we need to use Game~~\ref{blah}
   \begin{algorithm}[#1]%
   }
   {
   \end{algorithm}
   }

% ---------------------------------------------------------------------------

%Due to incompatibility between cryptocode and autonum, the following hack is needed. https://tex.stackexchange.com/questions/522666/incompatibility-between-cryptocode-and-autonum:
\expandafter\let\expandafter\savedflalignstar\csname flalign*\endcsname
\expandafter\let\expandafter\savedendflalignstar\csname endflalign*\endcsname
\AtBeginDocument{%
  \expandafter\let\csname flalign*\endcsname\savedflalignstar
  \expandafter\let\csname endflalign*\endcsname\savedendflalignstar
}


%Abstract:
%\newcommand{\ab}[1]{#1} \newcommand{\fv}[1]{}

%Full version:
\newcommand{\ab}[1]{} \newcommand{\fv}[1]{#1} %%


\ifnum\masterthesis=1
    \usepackage{setspace}
    \onehalfspacing
    \usepackage{fancyhdr}
    \pagestyle{fancy}
    \fancyhf{}
    \renewcommand{\headrulewidth}{0pt}
    \renewcommand{\headheight}{14pt}
    \chead{\thepage}
    
    \newcommand{\longunderline}{\underline{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }\ }
    
    \newenvironment{changemargin}[2]{%
        \begin{list}{}{%
        \setlength{\topsep}{0pt}%
        \setlength{\leftmargin}{#1}%
        \setlength{\rightmargin}{#2}%
        \setlength{\listparindent}{\parindent}%
        \setlength{\itemindent}{\parindent}%
        \setlength{\parsep}{\parskip}%
        }%
    \item[]}{\end{list}}
    
    \newcommand{\logoscale}{0.4}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% end macros

==> prudent contracts/macros.tex <==
%auto-ignore

\usepackage[draft=false]{hyperref}

\RequirePackage{etex}
\ifnum\sigconf=0\usepackage{authblk}\fi \usepackage{silence} %authbulk must loaded before the silence package!!
\usepackage[modulo]{lineno}
\usepackage{amsthm,amssymb,amsfonts,color,paralist,url,ifdraft,mathrsfs,thm-restate,comment,bbold,booktabs,fullpage}


\usepackage[utf8]{inputenc} \usepackage[autostyle=false, style=english]{csquotes} \MakeOuterQuote{"}

%csquotes after inputenc
\usepackage[T1]{fontenc}
\ifnum\sigconf=0
    \ifnum \shownomenclature=1
        \usepackage[refpage,prefix]{nomencl}
        \newcommand*{\nom}[3]{#2\nomenclature[#1]{#2}{#3}} 
        \makenomenclature
        % the following part makes the nomenclature to be a section rather than a section*. It also gives it a label. In the beginning, I had a solution which was based on the following url, but it stopped working, and that's why it is commented out: https://tex.stackexchange.com/questions/124608/how-to-format-the-name-of-a-nomenclature
        %\xpatchcmd{\thenomenclature}{
        %\section*{\nomname}}{% Replace it by the following
        %\section{\nomname}\label{sec:nomenclature}
        %}{\typeout{Success!}}{\typeout{Failure}}
        
        %since the previous solution didn't work, we simply redefine the command itself. See here for the original command: https://github.com/borisveytsman/nomencl/blob/master/nomencl.dtx
        \makeatletter
        \def\thenomenclature{%
            \providecommand*{\listofnlsname}{\nomname}%
      
        
            \section{\nomname}
            \label{sec:nomenclature}    
            \if@intoc\addcontentsline{toc}{section}{\nomname}\fi%
        
      
            \nompreamble
            \if@nomentbl
                \let\itemOrig=\item
                \def\item{\gdef\item{\\}}%
                \expandafter\longtable\expandafter{\@nomtableformat}
                \else
                \list{}{%
                  \labelwidth\nom@tempdim
                  \leftmargin\labelwidth
                  \advance\leftmargin\labelsep
                  \itemsep\nomitemsep
                  \let\makelabel\nomlabel}%
            \fi
        }
        \makeatother 
    \fi
    
    %\usepackage[draft=false,pageanchor]{hyperref}
    %\def\pagedeclaration#1{, \hyperlink{page.#1}{page\nobreakspace#1}} %This is needed for the nomenclature
    \usepackage{doi}

    \usepackage%[final]
    {graphicx}
\fi


 %\usepackage{mathtools} \mathtoolsset{showonlyrefs} %the mathtools way does not work nicely with sigconf. I *think* aotunum works in all cases.
%\ifdraft{\usepackage{showlabels}}{} %must be after use package{hyperref}.

%\usepackage[refpage,prefix]{nomencl} \newcommand*{\nom}[2]{#1\nomenclature{#1}{#2}} \makenomenclature
%\usepackage[displaymath,textmath,sections,graphics,floats]{preview}
%\RequirePackage{silence}
\WarningFilter{l3regex}{This package is obsolete }

\usepackage [ lambda,advantage , operators , sets , adversary , landau , probability , notions , logic ,ff, mm,primitives , events , complexity , asymptotics , keys]{cryptocode}
%the following commands are defined by crptocode. Define these ourselves if needed: \newcommand{\poly}{\mathrm{poly}} \newcommand{\prob}[1]{\Pr[ #1 ]} \newcommand{\norm}[1]{\left\| #1 \right\|} \newcommand{\RR}{\mathbb{R}} \newcommand{\FF}{\mathbb{F}} \newcommand{\CC}{\mathbb{C}} \newcommand{\NN}{\mathbb{N}}\DeclarePairedDelimiter\ceil{\lceil}{\rceil} \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\renewcommand{\verify}{\ensuremath{\mathsf{verify}}} 


%\renewcommand{\sfdefault}{phv}
%\renewcommand{\rmdefault}{ptm}

\ifdraft{\newcommand{\authnote}[3]{{\color{#3} {\bf  #1:} #2}}}{\newcommand{\authnote}[3]{}}
\newcommand{\note}[1]{{\color{red}#1}}
%Example for how this should be used, in main file:
\newcommand{\snote}[1]{\authnote{Shai}{#1}{purple}}


\newcommand{\CNOT}{\mathrm{CNOT}}
\newcommand{\defeq}{\stackrel{\mathrm{def}}{=}}

\newcommand{\const}{\mathrm{const}}

\newcommand{\bra}[1]{\langle #1 \vert}
\newcommand{\ket}[1]{\vert #1 \rangle}
\newcommand{\ketbra}[1]{\vert #1 \rangle \langle #1 \vert}
\newcommand{\braket}[2]{\langle #1 \vert #2 \rangle}
\newcommand{\conjugate}[1]{#1^{\dagger}}
\newcommand{\tensor}{\otimes}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\transpose}[1]{#1^{\mathsf{T}}}
\ifdraft{\linenumbers}{}

\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\E}{\mathbb{E}}

%\PreviewMacro*\onote
%\PreviewMacro*\nom
%\PreviewMacro*\ifdraft
%\DeclareMathOperator*{\E}{\scalerel*{\mathbb{E}}{\textstyle\sum}}


\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%document specific
\usepackage{algorithm,algorithmicx,algpseudocode}
\usepackage[normalem]{ulem}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sY}{\mathcal{Y}}
\newcommand{\sR}{\mathcal{R}}
\newcommand{\inj}{J}
\newcommand{\Es}[1]{\textsc{E}_{#1}}
\newcommand{\dset}{G}
\newcommand{\BQP}{\textsf{BQP}}
\renewcommand{\supp}{\textsc{Supp}}
\newcommand{\decrypt}{\ensuremath{\mathsf{decrypt}}}
\newcommand{\encrypt}{\ensuremath{\mathsf{encrypt}}}
\newcommand{\ds}{\ensuremath{\mathsf{DS}}}
\newcommand{\tm}{\ensuremath{\mathsf{TM}}}
\newcommand{\stamp}{
 {\mathchoice
  {\includegraphics[height=1.8ex]{RubberStamp}}
  {\includegraphics[height=1.8ex]{RubberStamp}}
  {\includegraphics[height=1.2ex]{RubberStamp}}
  {\includegraphics[height=0.9ex]{RubberStamp}}
 }
}
%\newcommand{\keygen}{\ensuremath{\mathsf{key\textit{-}gen}}}
%\newcommand{\sign}{\ensuremath{\mathsf{sign}}}
%\newcommand{\verify}{\ensuremath{\mathsf{verify}}}


\usepackage{tikz}
\usetikzlibrary{arrows,chains,matrix,positioning,scopes}
%
\makeatletter
\tikzset{join/.code=\tikzset{after node path={%
\ifx\tikzchainprevious\pgfutil@empty\else(\tikzchainprevious)%
edge[every join]#1(\tikzchaincurrent)\fi}}}
\makeatother
%
\tikzset{>=stealth',every on chain/.append style={join},
         every join/.style={->}}
\tikzstyle{labeled}=[execute at begin node=$\scriptstyle,
   execute at end node=$]
%
\ifnum\sigconf=0
    \usepackage[capitalise]{cleveref} %Incompatible with showonlyrefs
    \crefname{Game}{Game}{Games}
\fi

%\usepackage{autonum}%must be loaded after cleveref. Sometimes causes bugs. The alternative is incomaptible with cleveref:
 %\usepackage{mathtools} \mathtoolsset{showonlyrefs} %the mathtools way does not work nicely with sigconf. I *think* aotunum works in all cases. In any case, showonlyrefs does not work with cleveref.
\ifnum\sigconf=0
    \newtheorem{theorem}{Theorem} 
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{definition}[theorem]{Definition}
    \newtheorem{example}[theorem]{Example}
    \newtheorem{conjecture}[theorem]{Conjecture}
\fi 
  \newtheorem{claim}[theorem]{Claim}
  \newtheorem{fact}[theorem]{Fact}
  \newtheorem*{theorem*}{Theorem}
  \newtheorem*{lemma*}{Lemma}
  \newtheorem*{corollary*}{Corollary}
  \newtheorem*{proposition*}{Proposition}
  \newtheorem*{claim*}{Claim}
  
  \theoremstyle{definition}
  \newtheorem{openproblem}[theorem]{Open Problem}
  \theoremstyle{remark}
  \newtheorem{remark}[theorem]{Remark}

  \theoremstyle{plain}
  \renewcommand{\qedsymbol}{$\square$}

\theoremstyle{plain}
\newcounter{Game} 
\setcounter{Game}{0}
\newenvironment{game}[1][htb]
    {
    %\floatname{algorithm}{Game}% Update algorithm name
    %\refstepcounter{Game}%to call the Game pointer. Currently the problem is that caption command by default calls the algorithm pointer. For the moment we need to use Game~~\ref{blah}
   \begin{algorithm}[#1]%
   }
   {
   \end{algorithm}
   }

% ---------------------------------------------------------------------------

%Due to incompatibility between cryptocode and autonum, the following hack is needed. https://tex.stackexchange.com/questions/522666/incompatibility-between-cryptocode-and-autonum:
\expandafter\let\expandafter\savedflalignstar\csname flalign*\endcsname
\expandafter\let\expandafter\savedendflalignstar\csname endflalign*\endcsname
\AtBeginDocument{%
  \expandafter\let\csname flalign*\endcsname\savedflalignstar
  \expandafter\let\csname endflalign*\endcsname\savedendflalignstar
}


%Abstract:
%\newcommand{\ab}[1]{#1} \newcommand{\fv}[1]{}

%Full version:
\newcommand{\ab}[1]{} \newcommand{\fv}[1]{#1} %%


\ifnum\masterthesis=1
    \usepackage{setspace}
    \onehalfspacing
    \usepackage{fancyhdr}
    \pagestyle{fancy}
    \fancyhf{}
    \renewcommand{\headrulewidth}{0pt}
    \renewcommand{\headheight}{14pt}
    \chead{\thepage}
    
    \newcommand{\longunderline}{\underline{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }\ }
    
    \newenvironment{changemargin}[2]{%
        \begin{list}{}{%
        \setlength{\topsep}{0pt}%
        \setlength{\leftmargin}{#1}%
        \setlength{\rightmargin}{#2}%
        \setlength{\listparindent}{\parindent}%
        \setlength{\itemindent}{\parindent}%
        \setlength{\parsep}{\parskip}%
        }%
    \item[]}{\end{list}}
    
    \newcommand{\logoscale}{0.4}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% end macros
